Choice Models and Permutation Invariance: Demand Estimation in Differentiated Products Markets

Choice modeling is at the core of understanding how changes to the competitive landscape affect consumer choices and reshape market equilibria. In this paper, we propose a fundamental characterization of choice functions that encompasses a wide variety of extant choice models. We demonstrate how non-parametric estimators like neural nets can easily approximate such functionals and overcome the curse of dimensionality that is inherent in the non-parametric estimation of choice functions. We demonstrate through extensive simulations that our proposed functionals can flexibly capture underlying consumer behavior in a completely data-driven fashion and outperform traditional parametric models. As demand settings often exhibit endogenous features, we extend our framework to incorporate estimation under endogenous features. Further, we also describe a formal inference procedure to construct valid confidence intervals on objects of interest like price elasticity. Finally, to assess the practical applicability of our estimator, we utilize a real-world dataset from S. Berry, Levinsohn, and Pakes (1995). Our empirical analysis confirms that the estimator generates realistic and comparable own- and cross-price elasticities that are consistent with the observations reported in the existing literature.

==> Notes.tex <==


1. Informs 2023 workshop on data science, June 30, 2023 
https://connect.informs.org/discussion/cfp-the-2023-informs-workshop-on-data-science-1

2. MSOM Student Paper Competition, June 18, 2023
https://connect.informs.org/discussion/2023-msom-student-paper-competition-reminder-9

3. Jeff McGill Student Paper Award  (RMP), July 31st, 2023
https://connect.informs.org/rmp/awards/current-awards/student-award

----

https://platformanalytics.github.io/website//  Oct 15

Neurips workshop:
https://neurips.cc/virtual/2023/events/workshop

Causal Representation Learning. Oct 2,  https://crl-workshop.github.io/ 


---
To do: 
07.21 add figure 4 with raw IVs + add details of how we apply MLIV according to https://papers.ssrn.com/sol3/papers.cfm?abstract_id=3095039 - DONE


-- 
09.18
1. add J also include outside option - done
2. add in the beginning, not observed individual; observe aggregate   - done
3. instead of assumption 2 and 3, permutation invariant - done

4. add in appendix how each model is expressed in the form


5. show why endogeneity will fail the permutation invariance: assumption 1 fails, explain more.  - done
6. \gamma_0 is the true \gamma; add if you know the true model, then .....  - done
7. rename the z in the endogeneous section  - done
8. average effect of price change, say the object we are interested in ....   - done
9. some of the x, or p in the inference section, does not strengthen the price/ endogenous variabels   - done
10. first expectation, true population distribution of w_jt, then we have a empirical analog  - done
11. define \hat{\pi} before equation 6.  - done

12. non-parametric regression -> demand estimation - done
13. first say in a parametric estimation, inference, is root n consistent. Then however, if non-parametric, theta is not automatically consistent - done

14. we can divide by delta_p, because it is known and fixed  - done
15. if alpha or m correctly, then the moment function goes zero to explain the doubly robust -done
16. theorem 3, add a note, explain why line 2 to 3, line 1 to 2. - done



17. estimation explain how \gamma is estimated, put it inside, gamma is estimated used regression, (root n consistent); put step 1, 1a, then gamma hat, then 1b, pi_hat...=one
18. make connection to theorem 1, estimation, say pi is pho.. psi, move the first part of simulation to here. done
19. picture of neural network done - need to be further updated
20. step 3, cross fitting , use the word, add some citations. explain alpha, say, in practice, how we do....alpha we use the permutation invariance   done

add a method summary, summarize 3 things, on aggregate data, features of the model.   done



21. 4.1 rcl and mnl 4.1.1. data generation, 4.1.2. baseline models (make as bullet), add citation (Timoshenko, code is available, basket purchase, not over cite, improve, and also endogeneity)  -done 
22. utility, traditional.... but it is not necessary -done 
23. appendix number  - done 
24. N in each market   - done 
25. MNL add a footnote datageneration  - done 
26. say pi_hat in the table 
27. explain the number of observations - done 
28. in spite hyper parameter tuning; for the NP, the number of observations, put the J* k, for different models, one observation is a market; number of observations is xxx   - done 
29.  predictive performance (we first consider a basic thing, get pi_hat)  then inference  -done 
30. add the discussion of elasticitity, what is the value of permutation invariance, say our model with debiasing; elasticitifty at a given price, this is not debiase, it is not average. Next, in the inference, theta. elasticity is different.  
31. then other models, start with non-linear, cite with why non-linear utility become more common; until now, RCL is true model so it is / non-linear utility model 


- model misspecification. we are considering, start typical rcl are fully parametric, stylized, while fully NP no structure; however..... citation, (Lalit paper), two settings, using standard rcl and mnl, will not be able to catch up; we did not report inference because the intuition is similar 

- counterfactual analysis: NP cannot do, discuss what counterfactual are feasible. because of the permutation invariance. .... then we provide an example of minivan, new product 

advantage of our model, we do not need to specify, add the citation.


-----------
simulation of images. 
make slides 


----
get ready to share the code. 


----
09/20 
0. baseline, J-factorial, citation (aman), intuition, if not invariance. non-parametric cannot estimate beyond 10 products because data will not grow. before the last paragraph of the baseline; similar thing to non linear too. our permutation, phi2 on all the products, if there is variation in one product then can learn for other parametrics, similar to the parametric, logit. write a full paragraph. 
1. non-linear: consider only one feature x, on which we apply the following non-linear transformation g -- to define what is g; say we also estimate baseline models; for NP, will learn it directly; say something comparison to NP; - done 
2. paratheses put elasticity notation. full neural network also pick up. but still not pick up. W - done 

3. more inattention citation - hema, other models discussion, why inattention. - done
4. choice probabilty, for inattention part. for one product, another product.... -done
5. ranking, consideration; two-stage, some feature affect consideration.... then we focus on one ; 4.3 nicer title. broader choice behavior. show why the basic choice models fails, then ...  -done 
6. we again consider only one feature  -done
7. make inattention figure better in b&w, in figure, use the 5-product case so we can show NP. add some discussion of intuition instead of saying the "conclusion"  
8. counterfactual........one .... -done
9. 11th product is being added. 10 product + one outside option + 1 new product -done
10. bias and vairance --> MAE and RMSE  -done 
11. own price on demand - done 
12. once RCL then RCL. - done 
13. 50 samples --> 50 samples of draws - done 
14. standardize --> by z-scoring, substract mean, divide by done  - done 
15. automobiles - cars  - done 
16. blp, theta-0, prediction, make it more precise. table 14 is theta0
17. when saying elasticity, use the expression. - double check 
18. don's say the blue label, but the number.. line. - done 
19. conclusion, endogeneity and counterfactual
20. some references. 



discussion of inattention
inattention figure 

the market share ($\hat{\pi_{jt}}$), own-elasticity ($\hat{\frac{\partial \pi_{jt}}{\partial P_{jt}}}$) and cross-elasticity ($\hat{\frac{\partial \pi_{jt}}{\partial P_{k\neq j t}}}$)

